Learning to Generate Synthetic Data via Compositing

We present a task-aware approach to synthetic data generation. Our framework employs a trainable synthesizer network that is optimized to produce meaningful training samples by assessing the strengths and weaknesses of a `target' network. The synthesizer and target networks are trained in an adversarial manner wherein each network is updated with a goal to outdo the other. Additionally, we ensure the synthesizer generates realistic data by pairing it with a discriminator trained on real-world images. Further, to make the target classifier invariant to blending artefacts, we introduce these artefacts to background regions of the training images so the target does not over-fit to them. We demonstrate the efficacy of our approach by applying it to different target networks including a classification network on AffNIST, and two object detection networks (SSD, Faster-RCNN) on different datasets. On the AffNIST benchmark, our approach is able to surpass the baseline results with just half the training examples. On the VOC person detection benchmark, we show improvements of up to 2.7% as a result of our data augmentation. Similarly on the GMU detection benchmark, we report a performance boost of 3.5% in mAP over the baseline method, outperforming the previous state of the art approaches by up to 7.5% on specific categories.

==> introduction_original.tex <==
%auto-ignore
%<visesh>
%%%%%%%%% BODY TEXT
\section{Introduction}
\label{section:introduction}

Synthetic data generation is now increasingly utilized to overcome the burden of creating large
supervised datasets for training deep neural networks. A broad range of data synthesis
approaches have been proposed in literature, ranging from photo-realistic image
rendering~\cite{Krahenbuhl2018,playing,gul} and learning-based image
synthesis~\cite{Salimans2016,apple,Tran2017a} to methods for automating the data augmentation
process~\cite{Fawzi2016,Gupta2016a,Hauberg2016,Ratner2017}
by generating new example images from an existing training set.

For the task of object detection,
recent works have explored a compositing-based approach to data augmentation in which additional
training images are generated by inserting cropped foreground objects into novel
backgrounds~\cite{modeling-visual-context,cut-paste-learn}. The compositing approach, which is the
basis for this work, has two main advantages in comparison to image synthesis: 1) the domain gap
between the original and augmented image examples tends to be minimal (resulting primarily from
blending artifacts); and 2) the method is broadly-applicable, as it can be applied to any image
dataset with object annotations. The challenge with compositional approaches: is to be able to 1)
increase realism in the generated data; and to 2) ensure improvement in classifier performance when
fine-tuned on this data.

\begin{figure}
  \includegraphics[width=3.5in,height=1.5in]{figures/remteaser.pdf}
  \caption{We approach targeted data generation using synthesis-by-composition
  ~\cite{cut-paste-learn,modeling-visual-context,stgan}, by
  identifying and focusing on the weaknesses of a target classifier during generation.
  We iterate over cycles of data generation and classifier fine-tuning, 
  to eventually get an improved classifier.}
  \vspace{-0.25in}
\end{figure}
 
\begin{figure*}[h!]
	\centering
	\includegraphics[width=\textwidth]{figures/schematic-compact.pdf}
	\caption{
		{\bf Overview of our approach}: Our pipeline consists of three components: (i.) a
        synthesizer $\Theta$, (ii.) a target network $\mathcal{T}$, and (iii.) a natural image
        discriminator $\mathcal{D}$. The synthesizer composites a background image $b$ and a
        foreground mask $m$ to create a synthetic image $f$, after applying an affine transformation
        to $m$. The synthetic image $f$ is fed to the target network $\mathcal{T}$ 
        and a natural image discriminator $\mathcal{D}$, alongside real
        images $r$. While $\mathcal{D}$ is trained to differentiate between $r$ and $f$, the target
        network $\mathcal{T}$ is trained to accurately make predictions for both $r$ and $f$.
        The synthesizer $\Theta$ gets feedback from $\mathcal{T}$ and $\mathcal{D}$ and is 
        trained to generate transformations that yield realistic synthetic images that are hard 
        examples for $\mathcal{T}$.
        %Please
        %note that while in this case $\mathcal{T}$ is an object detector, it can also be an instance
        %detector or image classifier. 
	}
    \vspace{-0.2in}
	\label{fig:pipeline1}
\end{figure*} 
 
Traditional approaches to data augmentation have relied on task-specific data transformations that
preserve class labels~\cite{Tran2017a,autoaugment}, while more recent works
%Traditional approaches to synthesizing additional training data relied on sampling the parameter space
%of task-specific data transformations that preserve class labels. This is also referred to as data
%augmentation in literature. Recent works have 
extend data augmentation by generalizing the class
of image transforms~\cite{Hauberg2016} or even generating novel examples by
compositing~\cite{Ratner2017} different parts from real images.
Such approaches neither take into account the quality of synthetic data generated in terms of its
utility to improve classifier performance, nor modify their generation strategy as the target
classifier gets fine-tuned with generated data.
%These approaches do not take into account the quality of
%synthetic data generated in terms of its utility to improve the target network, and thus tend to be
%inefficient in terms of data volume required to achieve certain performance gains. Also, as the
%target network gets updated or fine-tuned to learn from this data, there is no feedback to the
%synthesis process to drive further improvement.

We argue that a synthetic data generation approach must have 3 important characteristics. It must
be a) \emph{efficient}: able to generate large, meaningful variations without generating excessive number
of samples, b) \emph{effective}: able to generate samples that can serve as hard positives for a 
target network and c) \emph{useful}: able to improve target network performance with generated data.
%We hypothesize that the synthetic data generation process can be made efficient by aligning the
%purpose of generating images with the goal of optimizing a given target network such as an image
%classification or detection network. 
Inspired by recent success of image synthesis via.
composition~\cite{Ratner2017}, we propose a \emph{smart} synthesizer network whose goal is to
produce valuable training data for the given task, that has all these characteristics. 
Our synthesizer network, which is trained in loop with the target network, is incentivized
to generate novel training examples that can \emph{fool} the target. 
A two player-game is setup between the synthesizer and the target network, 
such that the target is continuously updated to learn from the
synthetic data (along with original data), forcing the synthesizer to continuously adapt to the
target's strengths and weakness - analogous to hard example mining that is
sometimes employed in training networks by focusing on difficult positive and negative examples
during the training process~\cite{dpm}. 
%Hard example mining is typically limited to picking training
%samples from a given set and generally rely on simple ad-hoc metrics such as classification accuracy
%of the network being trained. 
In contrast to hard example mining, however, our approach can \emph{adaptively synthesize} 
training examples to potentially serve as hard positives for a target network at any given stage of
training.


\begin{figure*}[h!]
  \includegraphics[width=170mm,height=28mm]{figures/before-after-D.pdf}
	%\includegraphics[width=28mm,height=28mm]{figures/remsamples/figure1.jpg}
	%\includegraphics[width=28mm,height=28mm]{figures/remsamples/figure2.jpg}
	%\includegraphics[width=28mm,height=28mm]{figures/remsamples/figure3.jpg}
	%\includegraphics[width=28mm,height=28mm]{figures/remsamples/figure4.jpg}
	%\includegraphics[width=28mm,height=28mm]{figures/remsamples/figure5.jpg}
	%\includegraphics[width=28mm,height=28mm]{figures/remsamples/figure6.jpg}
	\caption{Importance of discriminator for synthesis of realistic adversarial examples. Composites created to fool SSD model~\cite{SSD-network} are much less realistic when generated \emph{without} discriminator (first 3 images) than they are when discriminator is used (last 3 images). \textbf{JMR: Can we tie this back to margin scores to quantify why realism matters?}}
	\label{fig:sleep_data_without_discriminator}
    \vspace{-0.25in}
\end{figure*}

\paragraph{Blending artifacts}
Composition based synthetic data generation methods have to usually with sensitivity to blending 
artifacts. To address the issues with blending, Dwibedi~\etal~\cite{cut-paste-learn}
employed $5$ different blending methods so that the target network does not latch on to a particular
blending artifact. Our solution to handling this issue is rather simple and intuitive. In addition
to positive examples, we create
synthetic negative examples by pasting foreground shaped cutouts from (background regions of) different images using the
same blending procedure. This makes the target network insensitive to any
blending artifacts around foreground objects, since the background images are plagued with similar
issues.
 
\paragraph{Realism and Context}
The generated synthetic data has to have sufficient realism and contextual information to improve
performance and
generalization of the target network~\cite{Divvala2009,Mottaghi2014,Oliva2007}. We accomplish this
by pairing the synthesizer with a
discriminator network that evaluates the synthetic image of the synthesizer to ensure that it conforms to the
distribution of real images. Implicitly, the discriminator also encodes contextual and affordance
information into the generated data, and thus obviates the need to construct explicit models of
context~\cite{modeling-visual-context,Divvala2009}.

The main contributions of our work are summarized below:
\begin{itemize}
    \item We present an novel image synthesizer CNN that learns to create composites 
	%\item We present a novel convolution neural network formulation for a image synthesizer that
    %  learns to create composite novel images by combining different foregrounds and backgrounds.
    %  The synthesizer learns to adaptively generates meaningful data for the target network as it
    %  is trained with goal of fooling the target. Similarly, target is continuously updated to learn
    %  from the synthesized examples, ensuring the synthesizer produces data relevant to current
    %  weakness of the target.
    specifically to \emph{fool} a target network. The synthesizer and target network are updated
    cyclically, until a convergence criteria is satisfied
	
	\item The target network is trained to be agnostic to blending artifacts by generating
      hallucinated similar artifacts in background images.
	
	\item A real image discriminator is employed to ensure the synthesizer geneates realistic and
      contextually salient images with appropriate affordances to help with generalization. 
      (Section~\ref{subsection:pascal_VOC}).
      % \TKTK{DO we have experiment for this?}
\end{itemize}

We apply our synthesis pipeline to demonstrate improvements on tasks such as digit classification on
the AffNist dataset, object localization using SSD~\cite{SSD-network} on Pascal
VOC~\cite{Pascal-voc}, and instance detection using Faster RCNN~\cite{FasterRCNN} on GMU
Kitchen~\cite{GMU-kitchen-dataset}  dataset. 
We demonstrate in these experiments, that our approach is a) \emph{efficient}: we can achieve similar performance for classifiers trained
with less than $50\%$ data than random sampling~(Section~\ref{subsec:affnist}), b) \emph{effective}: we
produce upto $50\%$ more hard positives compared to recent
approaches~\ref{subsec:hard_positive_mining}, and c) \emph{useful}: networks trained on our data achieve
upto $2.5\%$ improvement for person detection~(Section~\ref{subsection:pascal_VOC}) and over $3\%$
increase in mAP over all classes on the GMU kitchen dataset over
baseline~(Section~\ref{subsection:gmu_kitchen}).
%In our experiments on AFFNIST datasets, we demonstrate
%that we achieve the same performance with less that $50\%$ additional training data. Our
%experimental results demonstrate that our method can produce improvements in AP as much as 
%{\tt 2.5\%} over different IoU thresholds for person detection using the SSD model on the Pascal VOC
%benchmark. Similarly, for the problem of instance detection, we achieve a {\tt 3\%}
%increase in mAP over all classes on the GMU Kitchen dataset over baseline.
%Results show our network is \emph{efficient} (Section~\ref{subsec:affnist}), \emph{effective}
%(Section~\ref{subsec:hard_positive_mining}) and \emph{useful}
%(Section~\ref{subsection:pascal_VOC},\ref{subsection:gmu_kitchen}) 



%We compare with the state-of-the-art data generation approaches in all these cases~\cite{cut-paste-learn,modeling-visual-context}, and show superior performance.
%	 
%	in the sense that the training samples they produce are not optimized to improve the performance of the trained classifier, and significant domain expertise and finetuning is often needed to obtain good performance. In contrast, methods such as hard negative mining~\cite{shrivastava2016training} yield examples which are optimized to improve performance.
%
%A basic question which arises in any data augmentation approach is deciding what kinds of training images to synthesize. A classical approach is to draw random samples from the parameter space of task-specific data transformations that preserve the class labels. More recent works have explored automating the data augmentation process by generating novel examples through the composition~\cite{Ratner2017} or generalization~\cite{Hauberg2016} of image transforms. However, these approaches have the potential to be inefficient in the sense that the training samples they produce are not optimized to improve the performance of the trained classifier, and significant domain expertise and finetuning is often needed to obtain good performance. In contrast, methods such as hard negative mining~\cite{shrivastava2016training} yield examples which are optimized to improve performance. This paper addresses the challenge of optimizing the production of~\emph{hard positive} examples from an existing image training set using adversarial learning. While prior works on image composition~\cite{modeling-visual-context,cut-paste-learn} inspired our approach, these methods can fail to produce the hard positive examples that are needed for optimizing object detection performance, as illustrated in Fig.~\ref{fig:hardness_of_data} for SSD detection.

%%Data synthesis has gained increasing importance for training deep learning systems in the last few years. Primarily, such approaches have been used for either data augmentation, or for generating data to pre-train networks. While one reason for this is to avoid the problem of domain transfer from synthetic to real data, we argue that it is difficult to produce any \textbf{hard positives} from current approaches. This fact is illustrated in , where we compare {\tt SSD} scores on synthetic data generated by state-of-the-art algorithms~\cite{modeling-visual-context,cut-paste-learn}, to our approach. The lack of hard positives fundamentally limits the usefulness of synthetic data for training/improving a classifier and primarily restricts it to the role of a sidekick whose job is to take care of smaller issues, with real data doing the heavy lifting. Secondly, current synthetic data approaches generate data in an \textbf{objective free} manner: data is generated either using procedural approaches, or by using a system of rules that involve the various degrees of freedom associated with the scene and environment alone. However, none of the current approaches in literature, to the best of our knowledge, generate synthetic data \textbf{targeted at improving a desginated target}.

%Our approach to constructing hard positive examples from an existing training set is based on optimizing an objective function that \textsl{maximizes} misclassification, identifying examples that can fool the classifier into generating false negative labels. Such an approach runs the risk of producing examples which are unrealistic, and therefore don't improve generalization, as we show in Fig.~\ref{fig:ssd_qualitative_results} and discuss in Sec.~\ref{section:evaluation}. In line with recent
%work~\cite{stgan,xiao2018generating,zhao2017generating,pedestrian-synthesis-GAN}, we address this issue by adding a real/fake image discriminator in our pipeline to bias the data generation process towards \emph{realistic} synthetic examples. Such an approach has the benefit of avoiding the need to explicitly define image realism. Correct context is an important aspect of realism for object detection tasks~\cite{Mottaghi2014,Divvala2009,Oliva2007}. Our approach implicitly builds contextual information into the data generation process and obviates the need to construct explicit models of context~\cite{modeling-visual-context,Divvala2009}. This paper makes the following contributions:
%\begin{itemize}
%\item We present a novel method for synthesizing hard positive examples for image classification
%  tasks, based on cutting foreground objects and optimizing their placement into novel backgrounds.
%  Specifically, we propose to generate a set of {\bf transformations} that can be applied to the
%  foreground before creating a compsite with a given background image, while ensuring that the
%  composite image is highly likely to be misclassified by classifier/detector.
%\item We demonstrate through ablation studies that optimizing object placement and discriminating
%  between realistic and unrealistic images is crucial for effective generalization. We additionally
%  show that the data that we generate, on average, has more hard positives than current
%  approaches~\cite{cut-paste-learn,modeling-visual-context} in almost all categories and levels of
%  hardness.
%\item Our experimental results demonstrate that our method can produce accuracy gains of {\tt 2.5\%} in
%  standard datasets using the SSD classifier. In some classes like bicycles, we achieve an accuracy
%  gain of around {\tt 8\%}. Additionally, for the problem of instance detection, we achieve around {\tt
%  10\%}
%  increase in accuracy on the GMU Kitchen dataset. We compare with the state-of-the-art data
%  generation approaches in all these cases~\cite{cut-paste-learn,modeling-visual-context}, 
%  and show superior performance.
%%\item \textbf{Original contributions, need to merge:}
%%    \item We propose an approach to targeted synthetic data generation. Specifically, given two images (foreground and background), we propose to generate a set of \textbf{transformations} that can be applied to the foreground before doing a composite with the background, with the result having good chance of ''fooling'' a \textbf{target classifier}. This target could be an instance object detector, or a multi-class detector like SSD or blitznet. A typical foreground we use is segmentated objects in black background, while natural images are used for background.
%%    \item In order to do this effectively, our generator, compositor and target classifier are locked in a feedback loop. We back-propagate a form of loss called the \textbf{Half Inverse Cross Entropy} (HICE) loss, to enable the generator to learn parameters from a class of transformations that could be applied to foreground images.
%%    \item We add a real/fake image discriminator in this loop, and append a GAN loss to the HICE loss above, to enable the composite to look realistic. Implicitly, such an approach encourages the generator to learn context and affordance while placing the foreground in the composite.
%\item Finally, we give a probability grounded solution to the problem of \textbf{blending artifacts} reported in recent literature. We show that with the proposed solution, we do not need to have multiple blending options for creating composites. This has the advantage of making the blending part of our learning pipeline (using differentiable blending), giving us the ability to learn the alpha blending mask.
%\end{itemize}


%%the need to explicitly annotate additional image examples to guide data generation. Instead, we show that such an approach implicitly builds in contextual information 


%% We attempt to answer both of these questions with a targeted data generation approach that mines hard positives. We do this by devising an objective function for data generation that specifically aims at ''fooling'' a target classifier. Such an approach naturally produces hard positives as a consequence of the loss function, which tends to \textbf{maximize} misclassification. 
%By first
%taking an example of MNIST, we show that such an approach can quickly identify spaces of
%transformations that can be applied to data, such that the target classifier (MNIST digit classifier
%in this case) fails. This shows that our approach can mine hard positives. Next, we show that using
%the generated data for fine tuning the classifier and make can it robust to such transformations.
%This cycle can potentially be repeated until the classifier performance stops improving..
%</visesh>
%\subsection{Contributions}
%\label{subsection:contributions}




==> latexSuiteTemp0.tex <==
\label{subsec:affnist}
\begin{figure}[t!]
  \includegraphics[width=85mm,height=65mm]{figures/affNIST/result.png}
  \caption{Evaluation of ReM 1-1-0 on AffNIST data. Remember MNIST is the TC. Curves associated with
  { \tt ReM 1-1-0 EM} correspond to ReM model EM cycle. X-axis represents sleep cycles, and Y-axis
  represents accuracy obtained on AffNIST test data. Curves with { \tt Re-Init} show that the
  MNIST classifier was trained from scratch after every sleep cycle, before testing on AffNIST test
  data. Note how we are able to train better models, with lesser data. Also note how, given the
  correct data, even a 2 layer network is able to achieve over 90\% accuracy on AffNIST data.}
\end{figure}
 

\subsection{Hard Positive Mining}
\label{subsec:hard_positive_mining}

\begin{figure}[t!]
  \includegraphics[width=85mm,height=65mm]{figures/Hardness/comparison.png}
  \caption{Comparison between our approach and Cut-Paste-Learn, on the fraction of hard positives
  generated for the \emph{person} class. In the above plot, the X-axis represents classification accuracy of an {\tt SSD}
  network trained to ignore blending artifacts only. Both curves were plotted using the same amount

